Star formation at the smallest scales; A JWST study of the clump populations in SMACS0723

We present the clump populations detected in 18 lensed galaxies at redshifts 1 to 8.5 within the lensing cluster field SMACS0723. The recent JWST Early Release Observations of this poorly known region of the sky have revealed numerous point-like sources within and surrounding their host galaxies, undetected in the shallower HST images. We use JWST multiband photometry and the lensing model of this galaxy cluster to estimate the intrinsic sizes and magnitudes of the stellar clumps. We derive optical restframe effective radii from $<$10 to 100s pc and masses ranging from $\sim10^5$ to $10^9$ M$_{\odot}$, overlapping with massive star clusters in the local universe. The ages range from 1 Myr to 1 Gyr. We compare the crossing time to the age of the clumps and determine that between 45 and 60 % of the detected clumps are consistent with being gravitationally bound. The lack of Gyr old clumps suggest that the dissolution time scales are shorter than 1 Gyr. We see a significant increase in the luminosity (mass) surface density of the clumps with redshift. Clumps in galaxies at the reionisation era have stellar densities higher than massive clusters in the local universe. We zoom-in into single galaxies at redshift $<6$ and find for two galaxies, the Sparkler and the Firework, that their star clusters/clumps show distinctive colour distributions and location surrounding their host galaxy that are compatible with being accredited or formed during merger events. The ages of some of the compact clusters are between 1 and 4 Gyr, e.g., globular cluster precursors formed around 9-12 Gyr ago. Our study, conducted on a small sample of galaxies, shows the potential of JWST observations for understanding the conditions under which star clusters form in rapidly evolving galaxies.

==> observations.tex <==
\begin{table} 
 
\begin{tabular}{lllll} 
Filter & Exp time & Limit magnitude & Magnitude corrections & PSF FWHM \\ 
 &   [s] & AB mag & AB mag & [arcsec]  \\ 

\hline 
\hline 

HST F435W & 2,233 &  27.2 & &  \\ 
HST F606W & 2,289 &  27.6 & & \\ 
HST F814W & 2,529 &   27.1 & & \\ 
JWST F090W & 7,537  & 29.1 & -0.174 & 0.05  \\ 
HST F105W & 6,058 &  26.6  & &\\ 
HST F125W & 3,248 &  26.0  & &\\ 
HST F140W & 5,233 &  26.2  &  &\\ 
JWST F150W & 7,537  &  29.3 & -0.047 & 0.06 \\ 
HST F160W & 4,523 &  26.5 &  & \\ 
JWST F200W & 7,537  &  29.1 & -0.114 & 0.068 \\ 
JWST F277W & 7,537 &  29.1 & +0.223 & 0.11 \\ 
JWST F356W & 7,537 &  29.2  & +0.163 & 0.13 \\ 
JWST F444W & 7,537 &  29.0 & +0.162 & 0.14\\ 
\end{tabular} 
\caption{Photometric properties of the HST and JWST images. The HST filters limit magnitudes were measured by \citet{Coe2019}, and the JWST limits were measured in a PSF-like apperture in each filter. The last column gives the magnitudes corretions applied on the JWST filters and measured by \citet{adams2022}.}
\label{tab:table_observations} 
\end{table}

